On the Benefits of Traffic "Reprofiling'' -- The Single Hop Case

The need to guarantee hard delay bounds to traffic flows with deterministic traffic profiles, e.g., token buckets, arises in a number of network settings. Of interest are solutions that offer such guarantees while minimizing network bandwidth. The paper explores a basic building block towards realizing such solutions, namely, a single hop configuration. The main results are in the form of optimal solutions for meeting local deadlines under schedulers of varying complexity and therefore cost. The results demonstrate how judiciously modifying flows' traffic profiles, i.e., reprofiling them, can help simple schedulers reduce the bandwidth they require, often performing nearly as well as more complex ones.

==> one_hop.tex <==
\section{Solving the one-hop scenario}\label{sec:one_hop}
This section seeks to build insight into how to best solve problem \textbf{OPT} by exploring its simplest instantiation, a one-hop (single link) network as shown in \fig{fig:n_flow}. For further simplicity, we also assume that the $n$~flows sharing that network link are all connected through separate, dedicated access links of very high bandwidth. The (output) link bandwidth $R$ is then the quantity \textbf{OPT} aims to minimize while meeting the $n$~flows' deadlines. Further, the link is preceded by an infinite buffer and has capacity that exceeds the aggregate average arrival rate across all flows, so that the system is stable and lossless. Next, we characterize \textbf{OPT}'s solution (value of $R$) for different types of schedulers arbitrating flow transmissions on the shared link.  Of interest is the extent to which more sophisticated (expensive) schedulers translate into lower bandwidth values.

\input{one_hop_dynamic}
\input{one_hop_static}
\input{one_hop_shaper}
\input{one_hop_fifo}


